ProClosure: Hierarchical Room-Object Assignment using Progressive Boundary Closure from Monocular Video

A 3D scene graph groups objects into rooms. When a robot is asked to fetch an object from the kitchen, that grouping is what tells it where to look. An object recorded in the wrong room is not retrievable by a query naming the correct room. We introduce Progressive Boundary Closure, which recovers room layer from a monocular RGB video. A SLAM front end and an open-vocabulary segmenter supply a structural point cloud, camera trajectory and object tracks. The cloud is rasterised into a top-down map, rooms are recovered from it, and each object takes the room holding most of its extent. The difficulty lies in the map itself. Walls are recorded only where the camera looked, so a gap in the boundary may be a doorway or a stretch of wall that was never observed; nothing distinguishes the two. Prior methods treat both as passages, merging rooms that should remain separate. We observe that both require the same treatment: a room should not extend across either, so both are closed and need not be distinguished. Such an opening closes under a small amount of boundary growth, and few sightlines cross it, so points in different rooms rarely see one another. We use the first to recover rooms and the second to assign objects to them. Rooms are obtained by Progressively thickening the boundary inward and freezing each free-space region once it becomes enclosed, so every opening seals at its own scale rather than at a radius fixed in advance. Camera poses are used as seeds, which removes the sampling heuristic and makes the segmentation deterministic. Over 10 floors of 6 HM3D-Semantics scenes, scored against HOV-SG on identical top-down maps, we recover 74 rooms for 72 annotated regions (HOV-SG: 44), raising room F_1 from 0.741 to 0.890 at IoU 0.25 at some cost in precision, and object-to-room ARI from 0.488 to 0.696 (p=0.002, ahead on every floor).

==> figures/fig_pipeline.tex <==
% fig_pipeline.tex — Hero figure: pipeline overview (top) + closure sequence (bottom)
%
% Shape / colour conventions used in this figure (following common CV/ML paper practice):
%   Parallelogram (tape shape)  — data / artefact nodes (I/O)
%   Rectangle (rounded)         — processing / algorithm steps
%     · grey fill               — off-the-shelf / existing components
%     · blue fill               — canonical-projection step (bridge)
%     · rose/pink fill          — our contributions (highlighted)
%   Diamond                     — decision / branch point (none here; removed)
%   Arrows                      — solid = data flow; dashed = "zooms into" pointer
%
% Colour palette (all light shades for contrast):
%   Existing  : slate blue-grey  draw=blue!40!black!60, fill=blue!8!white
%   Bridge    : steel blue       draw=cyan!60!black,    fill=cyan!10!white
%   Contrib   : rose             draw=red!50!magenta!70!black, fill=red!8!magenta!5!white
%   Data pill : amber            draw=orange!80!black,  fill=yellow!20!white
%   Input/Out : light green      draw=green!50!black,   fill=green!8!white
%
% Required packages:
%   \usepackage{tikz}
%   \usetikzlibrary{arrows.meta, positioning, fit, backgrounds, calc,
%                   decorations.pathreplacing, shapes.geometric}

\begin{figure*}[t]
\centering
%% ── TOP SECTION: pipeline flowchart ──────────────────────────────────────────
\resizebox{\textwidth}{!}{%
\begin{tikzpicture}[
    >=Stealth,
    every node/.style={font=\small},
    % ── data artefacts: parallelogram (tape / data convention) ──
    data/.style={
        draw=orange!80!black, fill=yellow!30!white,
        shape=trapezium, trapezium left angle=80, trapezium right angle=100,
        minimum height=0.7cm, minimum width=2.0cm,
        align=center, font=\scriptsize\bfseries, inner sep=4pt
    },
    % ── input terminal: rounded rect, green ──
    io/.style={
        draw=green!55!black, fill=green!12!white,
        rounded corners=4pt,
        minimum height=1.0cm, minimum width=1.8cm,
        align=center, font=\small\itshape
    },
    % ── existing / off-the-shelf: rounded rect, slate blue-grey ──
    existing/.style={
        draw=blue!50!black!70, fill=blue!8!white,
        rounded corners=4pt,
        minimum height=1.15cm, minimum width=2.4cm,
        align=center, text width=2.2cm, font=\small
    },
    % ── canonical-projection bridge: rounded rect, steel blue ──
    bridge/.style={
        draw=cyan!70!black, fill=cyan!15!white,
        rounded corners=4pt,
        minimum height=1.15cm, minimum width=2.4cm,
        align=center, text width=2.2cm, font=\small
    },
    % ── our contributions: rounded rect, rose/pink ──
    contrib/.style={
        draw=red!55!magenta!80!black, fill=red!10!magenta!8!white,
        rounded corners=4pt, line width=0.9pt,
        minimum height=1.15cm, minimum width=2.4cm,
        align=center, text width=2.2cm, font=\small\bfseries
    },
    % ── arrows ──
    arr/.style={->, thick, black!70, line width=0.9pt},
    zoomar/.style={->, thick, dashed, black!45, line width=0.8pt},
    chanlabel/.style={font=\scriptsize\itshape, text=black!55},
]

% ── Input ──
\node[io] (video) at (0,0) {RGB\\Video};

% ── Reconstruction (existing) ──
\node[existing, right=0.9cm of video] (slam)
    {MASt3R-\\SLAM~{\scriptsize\cite{mast3rslam}}};

% ── Segmentation (existing) ──
\node[existing, right=0.85cm of slam] (sam3)
    {SAM3~{\scriptsize\cite{sam3}}\\{\scriptsize per-keyframe}};

% ── Structural data artefact ──
\node[data, above right=0.65cm and 1.0cm of sam3] (pw)
    {$\mathcal{P}_w$\\wall cloud};

% ── Canonical projection (bridge) ──
\node[bridge, right=0.85cm of pw] (align)
    {Gravity\,+\\Manhattan\\alignment};

% ── BEV map artefact ──
\node[data, right=0.85cm of align] (bev)
    {BEV map\\$W,\,F$};

% ── Progressive Closure (CONTRIBUTION) ──
\node[contrib, right=0.85cm of bev] (closure)
    {Progressive\\Closure\\{\scriptsize Sec.~\ref{sec:rooms}}};

% ── Object observations artefact ──
\node[data, below right=0.65cm and 1.0cm of sam3] (obs)
    {Object\\obs.};

% ── Voxel-IoS Tracker (existing) ──
\node[existing, right=0.85cm of obs] (tracker)
    {Voxel-IoS\\Tracker\\{\scriptsize Eq.~\eqref{eq:ios}}};

% ── Tracks artefact ──
\node[data, right=0.85cm of tracker] (tracks)
    {Tracks $\{o_j\}$\\centroids $\{c_j\}$};

% ── Rooms artefact (between closure and assign) ──
\node[data, below=0.5cm of closure] (rooms)
    {Rooms $\{\mathcal{R}_i\}$\\seeds $\{\mathcal{S}_i\}$};

% ── Visibility Agreement (CONTRIBUTION) ──
\node[contrib, right=0.85cm of rooms] (assign)
    {Visibility\\Agreement\\{\scriptsize Sec.~\ref{sec:assign}}};

% ── Assignment output artefact (end of pipeline, no scene graph box) ──
\node[data, right=0.85cm of assign] (outdata)
    {Object-to-room\\assignments $f$};

% ── Arrows ──
\draw[arr] (video) -- (slam);
\draw[arr] (slam) -- node[above, font=\tiny, yshift=1pt]{keyframes} (sam3);

% fork from SAM3
\draw[arr] (sam3.east) -- ++(0.3,0)
    |- node[chanlabel, pos=0.25, left, xshift=-1pt, yshift=1pt]{``wall''/``window''} (pw.west);
\draw[arr] (sam3.east) -- ++(0.3,0)
    |- node[chanlabel, pos=0.25, left, xshift=-1pt]{other prompts} (obs.west);

% structural path
\draw[arr] (pw)    -- (align);
\draw[arr] (align) -- (bev);
\draw[arr] (bev)   -- (closure);

% object path
\draw[arr] (obs)     -- (tracker);
\draw[arr] (tracker) -- (tracks);

% convergence into assignment
\draw[arr] (closure) -- (rooms);
\draw[arr] (rooms)   -- (assign);
\draw[arr] (tracks.east) -- ++(0.5,0)
    |- ([yshift=-0.18cm]assign.south east);
\draw[arr] (assign) -- (outdata);

% ── Background shading bands ──
\begin{scope}[on background layer]
    % existing components — pale blue-grey
    \node[fill=blue!5!white, draw=blue!25, dashed, rounded corners=6pt,
          inner sep=9pt,
          fit=(slam)(sam3)(pw)(align)(obs)(tracker),
          label={[font=\scriptsize\itshape, text=blue!50!black]{below left:existing components}] {};
          
    % bridge step — pale cyan
    \node[fill=cyan!6!white, draw=cyan!30, dashed, rounded corners=6pt,
          inner sep=9pt, fit=(bev),
          label={[font=\scriptsize\itshape, text=cyan!50!black]{below:canonical projection}] {};
    % contributions — pale rose
    \node[fill=red!4!magenta!4!white, draw=red!40!magenta!50, dashed,
          rounded corners=6pt, inner sep=9pt,
          fit=(closure)(rooms)(assign),
          label={[font=\scriptsize\itshape, text=red!50!magenta!70!black]{above left:our contributions}] {};
\end{scope}

\end{tikzpicture}%
}% end resizebox — pipeline row

\vspace{1.2cm}   % ← generous gap between pipeline and results row

%% ── BOTTOM SECTION: closure sequence with real images ───────────────────────
\newlength{\panelW}
\setlength{\panelW}{0.155\textwidth}   % each panel width

\resizebox{\textwidth}{!}{%
\begin{tikzpicture}[
    >=Stealth,
    every node/.style={font=\scriptsize},
    panelborder/.style={draw=black!35, line width=0.6pt},
    paneltitle/.style={font=\scriptsize\bfseries, text=black!80},
    arr/.style={->, thick, black!50, line width=0.8pt},
    zoomar/.style={->, thick, dashed, red!50!magenta!60, line width=0.9pt},
]

% Panel spacing
\def\panelgap{0.18}     % cm gap between panels
\def\pw{3.8}            % panel width in cm
\def\ph{2.4}            % panel height in cm

% Compute x positions
\pgfmathsetmacro{\xb}{\pw+\panelgap}
\pgfmathsetmacro{\xc}{2*(\pw+\panelgap)}
\pgfmathsetmacro{\xd}{3*(\pw+\panelgap)}
\pgfmathsetmacro{\xe}{4*(\pw+\panelgap)}

% ── Panel (a): clusters — final room clusters ──
\node[panelborder, minimum width=\pw cm, minimum height=\ph cm,
      anchor=north west] (pa) at (0,0)
    {\includegraphics[width=\pw cm, height=\ph cm, keepaspectratio=false]%
     {figures/clusters.png}};
\node[paneltitle, anchor=south, yshift=2pt] at (pa.north)
    {(a) Rooms $\{\mathcal{R}_i\}$};
\node[font=\tiny\itshape, text=black!50, anchor=north, yshift=-2pt] at (pa.south)
    {5 rooms, seeds at $p^{\mathrm{init}}$};

% ── Panel (b): iter_001 — Raw BEV, all seeds active ──
\node[panelborder, minimum width=\pw cm, minimum height=\ph cm,
      anchor=north west] (pb) at (\xb cm, 0)
    {\includegraphics[width=\pw cm, height=\ph cm, keepaspectratio=false]%
     {figures/iter_001.png}};
\node[paneltitle, anchor=south, yshift=2pt] at (pb.north)
    {(b)~$t=1$: seeds placed};
\node[font=\tiny\itshape, text=black!50, anchor=north, yshift=-2pt] at (pb.south)
    {all 48 seeds active};

% ── Panel (c): iter_009 — mid dilation, rooms separating ──
\node[panelborder, minimum width=\pw cm, minimum height=\ph cm,
      anchor=north west] (pc) at (\xc cm, 0)
    {\includegraphics[width=\pw cm, height=\ph cm, keepaspectratio=false]%
     {figures/iter_009.png}};
\node[paneltitle, anchor=south, yshift=2pt] at (pc.north)
    {(c)~$t=9$: walls thicken};
\node[font=\tiny\itshape, text=black!50, anchor=north, yshift=-2pt] at (pc.south)
    {narrow gaps closing};

% ── Panel (d): iter_017 — partial sealing 19/48 frozen ──
\node[panelborder, minimum width=\pw cm, minimum height=\ph cm,
      anchor=north west] (pd) at (\xd cm, 0)
    {\includegraphics[width=\pw cm, height=\ph cm, keepaspectratio=false]%
     {figures/iter_017.png}};
\node[paneltitle, anchor=south, yshift=2pt] at (pd.north)
    {(d)~$t=17$: sealing};
\node[font=\tiny\itshape, text=black!50, anchor=north, yshift=-2pt] at (pd.south)
    {19/48 frozen at own scale};

% ── Panel (e): rays — sightlines for object assignment ──
\node[panelborder, minimum width=\pw cm, minimum height=\ph cm,
      anchor=north west] (pe) at (\xe cm, 0)
    {\includegraphics[width=\pw cm, height=\ph cm, keepaspectratio=false]%
     {figures/rays.png}};
\node[paneltitle, anchor=south, yshift=2pt] at (pe.north)
    {(e) Sightlines};
\node[font=\tiny\itshape, text=black!50, anchor=north, yshift=-2pt] at (pe.south)
    {rays pruned across rooms};

% ── Thin separator arrow between panels (a–d) ──
\foreach \from/\to in {pa/pb, pb/pc, pc/pd}{
    \draw[arr] ([xshift=1mm]\from.east) -- ([xshift=-1mm]\to.west);
}

% ── Dashed gap: closing to assignment ──
\draw[arr, dashed] ([xshift=1mm]pd.east) -- ([xshift=-1mm]pe.west);

% ── Timeline brace under panels (a)–(d) ──
\draw[decorate, decoration={brace, amplitude=5pt, mirror},
      thick, blue!50!black!60]
    ([yshift=-0.55cm]pa.south west) -- ([yshift=-0.55cm]pd.south east)
    node[midway, below=6pt, align=center, font=\scriptsize,
         text=blue!60!black]
    {progressive closure — each room seals at its own scale (Eq.~\eqref{eq:freeze})};



\end{tikzpicture}
}

\caption{%
\textbf{System overview and progressive closure.}
\emph{Top (pipeline):}
A monocular RGB video is processed by MASt3R-SLAM~\cite{mast3rslam} and SAM3~\cite{sam3}.
Structural masks (wall, window) accumulate into~$\mathcal{P}_w$; other masks become object observations tracked by voxel-IoS matching.
$\mathcal{P}_w$ is gravity- and Manhattan-aligned into a binary top-down map~$(W,F)$.
Our two contributions (pink boxes) follow: \emph{progressive boundary closure} recovers room seeds~$\{\mathcal{S}_i\}$ (Sec.~\ref{sec:rooms}), and \emph{visibility agreement} assigns each object to a room (Sec.~\ref{sec:assign}).
\emph{Bottom (closure sequence, scene \texttt{00890}):}
(a)~Final five rooms coloured by cluster at original seed positions.
(b)~Initial BEV with 48 witness seeds placed in free space.
(c)~After 9 iterations, walls have thickened and rooms are separating.
(d)~By iteration 17, first rooms seal and seeds lock, protected from further growth.
(e)~Seed sightlines after cross-cluster pruning, used for object-to-room assignment.}%
\label{fig:pipeline}
\end{figure*}


==> preamble.tex <==

\makeatletter

%% ---------------------------------------------------------------------
%% 1. Encoding / fonts   (acmart sets these up itself)
%% ---------------------------------------------------------------------
\@ifclassloaded{acmart}{}{%
  \usepackage[utf8]{inputenc}
  \usepackage[T1]{fontenc}
}

%% ---------------------------------------------------------------------
%% 2. Math
%% ---------------------------------------------------------------------
\usepackage{amsmath}
%% acmart's maths fonts already provide the amssymb/amsfonts symbols and
%% define \Bbbk themselves; loading them again is a "already defined" error.
\@ifclassloaded{acmart}{}{%
  \usepackage{amssymb}
  \usepackage{amsfonts}
}

%% ---------------------------------------------------------------------
%% 3. Graphics
%% ---------------------------------------------------------------------
\usepackage{graphicx}
\graphicspath{{figures/}{figures/workflow/}{figures/bev/}{figures/qualitative/}}

%% ---------------------------------------------------------------------
%% 4. Tables
%% ---------------------------------------------------------------------
\usepackage{booktabs}
\usepackage{array}
\usepackage{multirow}
\usepackage{tabularx}
\newcolumntype{Y}{>{\centering\arraybackslash}X}

%% adjustbox gives "max width=" -- shrink-to-fit that never ENLARGES.
%% The tables use it instead of \resizebox{\columnwidth}{!}, which in the
%% one-column arXiv layout would scale them up ~2x (see README).
\usepackage{adjustbox}
\newenvironment{fittable}
  {\begin{adjustbox}{max width=\linewidth}}
  {\end{adjustbox}}


%% ---------------------------------------------------------------------
%% 5. Floats / captions / lists
%%    acmart forbids the caption package and supplies its own.
%% ---------------------------------------------------------------------
\usepackage{float}
\@ifclassloaded{acmart}{}{\usepackage{caption}}
\usepackage{enumitem}

%% ---------------------------------------------------------------------
%% 6. Algorithms   (algorithm.sty builds on float, so load it after)
%% ---------------------------------------------------------------------
\usepackage{algorithm}
\usepackage{algpseudocode}

%% ---------------------------------------------------------------------
%% 7. Colour + TikZ   (must come before hyperref)
%% ---------------------------------------------------------------------
\usepackage{xcolor}
\@ifpackageloaded{colortbl}{}{\usepackage{colortbl}}

\definecolor{oursgrey}{rgb}{0.93,0.93,0.96}       % ~black!8; prints and photocopies cleanly
\newcommand{\ourrow}{\rowcolor{oursgrey}}
\newcommand{\oc}{\cellcolor{oursgrey}}
\newcommand{\snd}[1]{\underline{\smash{#1}}}

\usepackage{pifont}
\newcommand{\cmark}{\textcolor{green!55!black}{\ding{51}}}
\newcommand{\xmark}{\textcolor{red!75!black}{\ding{55}}}

\usepackage{tikz}
% \usetikzlibrary{arrows.meta, positioning, fit, backgrounds, calc,
%                 decorations.pathreplacing, shapes.geometric, chains, spy}
\usetikzlibrary{arrows.meta, positioning, fit, backgrounds, calc, shapes, decorations}
%% ---------------------------------------------------------------------
%% 8. Microtypography
%% ---------------------------------------------------------------------
\usepackage{microtype}
%% ---------------------------------------------------------------------
%% 9. Citations + hyperlinks  (LOAD LAST -- both guarded, acmart owns them)
%% ---------------------------------------------------------------------
\@ifpackageloaded{natbib}{}{\usepackage[numbers]{natbib}}
\@ifpackageloaded{hyperref}{}{\usepackage[colorlinks=true]{hyperref}}

%% Sky-blue links (Okabe-Ito sky, darkened for print legibility)
\definecolor{skylink}{HTML}{2E86C8}
\hypersetup{colorlinks=true, allcolors=skylink}

%% =====================================================================
%%  SHARED FIGURE STYLES
%%  Every TikZ figure in 1_main-content.tex and 2_supp-content.tex
%%  draws on these, so the three diagrams cannot drift apart visually.
%%  Okabe-Ito colour-blind-safe palette.
%% =====================================================================
\providecolor{oiOrange}{HTML}{E69F00}
\providecolor{oiSky}{HTML}{56B4E9}
\providecolor{oiGreen}{HTML}{009E73}
\providecolor{oiBlue}{HTML}{0072B2}
\providecolor{oiVermillion}{HTML}{D55E00}
\providecolor{oiPurple}{HTML}{CC79A7}
\providecolor{oiGrey}{HTML}{999999}

\tikzset{
  every node/.style = {font=\footnotesize},
  proc/.style       = {rectangle, rounded corners=1pt, draw=oiGrey!80!black,
                       fill=oiGrey!12, minimum height=5mm, inner xsep=3pt, align=center},
  ours/.style       = {rectangle, rounded corners=1pt, draw=oiPurple,
                       fill=oiPurple!15, minimum height=5mm, inner xsep=3pt, align=center},
  data/.style       = {trapezium, trapezium left angle=70, trapezium right angle=110,
                       draw=oiSky!80!black, fill=oiSky!12, inner xsep=2pt, align=center},
  store/.style      = {cylinder, shape border rotate=90, aspect=0.25,
                       draw=oiBlue!80!black, fill=oiBlue!12, align=center},
  term/.style       = {rectangle, rounded corners=3pt, draw=oiGreen!80!black,
                       fill=oiGreen!12, align=center},
  flow/.style       = {-{Stealth[length=2mm]}, draw=black!70, rounded corners=2pt},
  flowdash/.style   = {-{Stealth[length=2mm]}, draw=black!45, dashed,
                       dash pattern=on 2pt off 1.5pt, rounded corners=2pt},
  grp/.style        = {draw=oiBlue!55, dashed, dash pattern=on 2pt off 1.5pt,
                       rounded corners=3pt, inner sep=5pt, fill=oiBlue!05},
  grpours/.style    = {draw=oiPurple, dashed, dash pattern=on 2pt off 1.5pt,
                       rounded corners=3pt, inner sep=4pt, fill=oiPurple!08},
  grplab/.style     = {font=\scriptsize\scshape, anchor=north west, text=oiBlue!65!black},
  grplabours/.style = {font=\scriptsize\scshape, anchor=north west, text=oiPurple!80!black},
  dflow/.style      = {-{Stealth[length=1.9mm]}, draw=black!62,
                       dash pattern=on 1pt off 1.1pt, line width=.55pt, rounded corners=1.5pt},
  thumb/.style      = {inner sep=0, outer sep=0},
  sublab/.style     = {font=\scriptsize, text=black!70},
}

%% =====================================================================
%%  CLASS SHIMS
%%  Two commands in the content files exist only under acmart.  These
%%  make the same content compile unchanged under article + arxiv.sty.
%% =====================================================================

%% The wide title-spanning teaser.  1_main-content.tex wraps it in
%% \begin{proteaser} ... \end{proteaser} instead of a class-specific
%% environment, so the same content file compiles under both classes.
%%
%% A full-width float is used in BOTH builds, deliberately.  acmart's
%% own \begin{teaserfigure} must appear BEFORE \maketitle, but the teaser
%% lives inside 1_main-content.tex, which is read AFTER \maketitle in
%% every main file -- so acmart would reject it there.  A figure* spans
%% both columns and floats to the top of page 1, which is where the
%% teaser sat anyway.
%%
%% To get acmart's true teaser back for an ACM camera-ready: swap the two
%% branches below AND move the proteaser block out of 1_main-content.tex
%% into main.tex, above \maketitle.
\@ifclassloaded{acmart}
  {\newenvironment{proteaser}{\begin{figure*}[!t]}{\end{figure*}}}
  {\newenvironment{proteaser}{\begin{figure*}[!t]}{\end{figure*}}}

%% acmart requires \Description{} on every float for accessibility.
%% \providecommand leaves acmart's real one alone and gives every other
%% class a harmless no-op, so the content files never need an \ifacm.
\providecommand{\Description}[1]{}

\makeatother

%% =====================================================================
%%  SUPPLEMENT TOGGLE
%%
%%  \supptrue   -> one PDF: body + references + full appendix   (arXiv)
%%  \suppfalse  -> body + references only, appendix uploaded separately
%%                 (conference submission with a page limit)
%%
%%  \suppref / \supprefp render a pointer into the appendix that works
%%  in BOTH builds: a live \ref when the appendix is present, a manual
%%  letter when it is not.
%%    #1 = manual appendix letter, used only in the \suppfalse build
%%    #2 = the real label, live only in the \supptrue build
%% =====================================================================
\newif\ifsupp
\supptrue

\newcommand{\suppref}[2]{\ifsupp Appendix~\ref{#2}\else the supplementary, Sec.~#1\fi}
\newcommand{\supprefp}[2]{\ifsupp Appendix~\ref{#2}\else supplementary, Sec.~#1\fi}

%% ---------------------------------------------------------------------
%% Layout tuning applied to every build
%% ---------------------------------------------------------------------
\raggedbottom
\emergencystretch=1.2em

%% arxiv.sty ships with a hardcoded running head, "PRIME AI paper" --- a
%% leftover from whoever built that style file.  Overriding it here rather
%% than editing arxiv.sty keeps the downloaded style file pristine.
%% acmart does not use fancyhdr, hence the guard.
%% >>> Change the text below if you want a different running head.
\makeatletter
\@ifclassloaded{acmart}{}{\rhead{\textit{ProClosure}}}
\makeatother

% This is the preamble file
% \newenvironment{teaserfigure}{\begin{figure*}[t]}{\end{figure*}}

